Verification Challenge: Fractional Cascading for Multi-Nuclide Grid Lookup

We present a verification challenge based on the fractional cascading (FC) technique for accelerating repeated searches across a collection of sorted arrays. The specific context is nuclear cross section lookup in a simulation code, where a material consists of many nuclides, each with its own sorted energy grid. A naive search performs a binary search in each array individually. The FC-based cascade grid structure reduces this cost by performing a single binary search followed by constant-time refinements. The challenge consists of verifying the correctness of the FC algorithm with respect to the naive approach and validating its structural properties.

==> eptcsdata.tex <==
\providecommand{\firstpage}{106}
\providecommand{\publicationstatus}{S.F.\ Siegel and G.\ Gopalakrishnan (Eds.):\\
International Workshop on Verification of\\
Scientific Software (VSS 2025)\\
EPTCS 432, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.432.12}{10.4204/EPTCS.432.12}}

